BIOT: Cross-data Biosignal Learning in the Wild

Biological signals, such as electroencephalograms (EEG), play a crucial role in numerous clinical applications, exhibiting diverse data formats and quality profiles. Current deep learning models for biosignals are typically specialized for specific datasets and clinical settings, limiting their broader applicability. Motivated by the success of large language models in text processing, we explore the development of foundational models that are trained from multiple data sources and can be fine-tuned on different downstream biosignal tasks. To overcome the unique challenges associated with biosignals of various formats, such as mismatched channels, variable sample lengths, and prevalent missing values, we propose a Biosignal Transformer (\method). The proposed \method model can enable cross-data learning with mismatched channels, variable lengths, and missing values by tokenizing diverse biosignals into unified "biosignal sentences". Specifically, we tokenize each channel into fixed-length segments containing local signal features, flattening them to form consistent "sentences". Channel embeddings and {\em relative} position embeddings are added to preserve spatio-temporal features. The \method model is versatile and applicable to various biosignal learning settings across different datasets, including joint pre-training for larger models. Comprehensive evaluations on EEG, electrocardiogram (ECG), and human activity sensory signals demonstrate that \method outperforms robust baselines in common settings and facilitates learning across multiple datasets with different formats. Use CHB-MIT seizure detection task as an example, our vanilla \method model shows 3\% improvement over baselines in balanced accuracy, and the pre-trained \method models (optimized from other data sources) can further bring up to 4\% improvements.

==> relatedworks.tex <==
\section{Related Works}

\noindent {\bf Model Architectures for Biosignals.} Biological signals (e.g., EEG, ECG, EMG) are usually recorded in multiple channels simultaneously at a high sampling rate (e.g., 256Hz). Previous biosignal learning methods involve hand-crafted features \cite{yuan2011epileptic,alzoubi2009classification} and traditional methods, such as support vector machine (SVM). To learn biosignal embeddings, existing DL models \cite{craik2019deep} mostly apply 1D convolutional neural networks (CNN) on the raw signals \citep{jing2023development,nagabushanam2020artifact,dar2020cnn}, or apply short-time Fourier transform (STFT) as preprocessing and use 2D CNN models on the spectrogram \citep{yang2022atd,kim2020study,cui2020eeg}, or split the signal into sessions and then apply a CNN session encoder plus a downstream sequence model (e.g, Transformer or RNN) \citep{zhang2019cnnlstm,biswal2018expert,jing2020development,almutairi2021detection} for capturing the temporal information. Some other models consider ensemble learning and feature fusion from multiple encoders \citep{li2022motor}. Recent models also encode the spatial (between channels) and temporal (within channels) features \citep{lawhern2018eegnet} by multi-level transformer \citep{song2021transformer,liu2021transformers}.

\noindent {\bf Supervised Learning on EEG.} Supervised learning approaches have been widely employed to analyze and classify EEG samples for understanding patients' physiological status, such as automatic sleep stage classification \citep{phan2022automatic,sekkal2022automatic,huang2022improved,zhao2022evaluation,yangmanydg}, sleep apnea detection \citep{mahmud2020sleep,wang2022bi,vimala2019intelligent,locharla2022eeg}, epileptic seizure detection \citep{jing2023development,yangmanydg,hussein2018epileptic,ahmad2022eeg,abdelhameed2021deep}, motor imagery classification \citep{altaheri2021deep,al2021deep,amin2019deep,dai2020hs,wang2018lstm,dai2019eeg}, emotion analysis and recognition \citep{dadebayev2022eeg,zhang2020investigation,bazgir2018emotion,topic2021emotion,doma2020comparative}.

\noindent {\bf Unsupervised Learning on EEG.} Unsupervised learning leverages the vast amount of unlabeled data for training encoder models. Existing works optimize unsupervised EEG encoders by several techniques, including contrastive learning \citep{zhang2022self,kostas2021bendr,shen2022contrastive,jiang2021self,cheng2020subject,yang2021self,banville2021uncovering} and autoencoders \citep{wen2018deep,sun2019unsupervised,yildiz2022unsupervised,qiu2018denoising,li2022novel}.

Given the advancement in biosignal learning, most existing models assume the input signals has fixed formats (fixed channels and duration without missing), which limits the model application scope. This paper for the first time proposes a generic biosignal encoding model \method to accommodate variable-format biosignals. We use EEG signals and tasks as exmaples in the experiments.
